The use of statistical methods for the search for new physics at the LHC (in Russian)

We review statistical methods used for the search for new physics at LHC.

==> ch8/chap8_full.tex <==
%\usepackage[koi8-r]{inputenc}

\newpage

\section{Статистическое программное обеспечение в задачах физики высоких энергий}

Данный раздел подготовлен при участии И.В.~Ажиненко и В.В.~Смирновой.

\subsection{Обзор основных пакетов}

Базовым инструментарием для решения задач физики высоких энергий является система 
программ ROOT~\cite{ROOT}. ROOT -- пакет объектно-ориентированных программ 
и библиотек, разработанный в ЦЕРН. Проект базируется на свободном программном 
обеспечении. Наряду со специальными средствами программирования и стандартных 
математических вычислений, ROOT обеспечивает пользователя средствами для построения и 
анализа гистограмм и графиков функций, средствами фитирования и подбора теоретических 
и экспериментальных зависимостей, инструментарием для проведения статистического 
(в том числе многофакторного) анализа данных~\cite{ROOTstat}.

Большинство программных наработок, по возможности, либо встраиваются в ROOT, либо являются 
надстройкой над ROOT, то есть базируются на ROOTовских библиотеках.
Проводятся работы по совмещению и/или по созданию интерфейса между
пакетом ROOT и астрофизическим языком и оболочкой для статистических
расчетов и построения графиков R~\cite{R}. 

Надстройкой над ROOT является пакет программ RooFit~\cite{RooFit}. 
RooFit это инструментарий для моделирования ожидаемых распределений событий
в физическом анализе. Пакет был изначально ориентирован на эксперимент BaBar.
Пакет удобен для быстрого Монте Карло розыгрыша событий 
и статистической обработки полученых распределений. Со временем он стал универсальным и 
базовым для пакетов, расширяющих его возможности, например, 
RooStats~\cite{RooStats}.  
 
Байесовская парадигма реализована в пакете программ BAT - 
The Bayesian Analysis Toolkit~\cite{BAT}. 
Анализ базируется на теореме Байеса и использует Монте Карло
моделирование Марковских цепей. Это позволяет строить апостериорное 
распределение вероятностей, производить оценивание параметров, строить 
доверительные интервалы, осуществлять перенос неопределенностей. 

Много внимания Статистические группы экспериментов уделяют статистическим 
пакетам многомерного анализа. Было проведено несколько мини-совещаний по 
данной тематике, например,  Miniworkshop on Statistical Tools (2008) 
DESY~\cite{MWST}, CMS tutorials on Multivariate Analysis 
Methods (2007) CERN~\cite{CMSMVA}. Здесь можно 
выделить пакет TMVA - Toolkit for MultiVariate Data Analysis~\cite{TMVA}. 
Данный инструментарий также встроен в среду ROOT и ориентирован на использование 
многомерных классификационных алгоритмов для решения широкого спектра задач.  
Для решения задач физики высоких энергий и астрофизики также разрабатывается пакет 
StatPatternRecognition (SPR)~\cite{SPR}. Оба пакета имеют как перекрывающиеся, 
так и дополняющие друг друга возможности. 
Интересной новой разработкой является система поддержки принятия
решений при выборе переменных в многомерном анализе и уменьшения 
размерности задачи PARADIGM~\cite{PARADIGM}. 


\subsection{Проект RooStats}

Для анализа экспериментальных данных коллабораций CMS и ATLAS разрабатывается  
проект RooStats~\cite{RooStats}, основанный на комплексе программ 
ROOT~\cite{ROOT}. Главные цели проекта  
\begin{itemize}
\item предоставить пользователю компьютерные программы с наиболее распространенными 
статистическими методами, которые применяются при анализе данных в физике высоких энергий, 
\item стандартизовать используемые методы для легкого сравнения результатов полученных 
разными группами и разными экспериментами. 
\end{itemize}


RooStats использует три наиболее распространенных подхода в статистике: 

\begin{enumerate}
\item частотный подход, 
\item метод максимального правдоподобия, 
\item Байесовский подход. 
\end{enumerate}

Заметим, что программа $RooStats$ постоянно развивается, совершенствуется и,   
на сегодняшний день, она содержит программы, позволяющие решать следующие задачи:

\begin{enumerate}
\item Точечная оценка для определения наилучшего в некотором смысле (например оценки с 
минимальной дисперсией или наиболее вероятные значения) значения параметра. 
\item Определение доверительного интервала: областей параметров функции распределения, 
не противоречащих наблюдаемым данным. 
\item Проверка гипотез: оценка значения вероятности $p$ для одной или нескольких 
гипотез (значимость). 
\item Оценка качества фита -- количественное определение насколько хорошо модель описывает 
данные.
\end{enumerate}

Программа RooStats написана на языке $C++$ и содержит следующие классы, 
позволяющие решать эти задачи. 

\begin{itemize}
\item[-] ProfileLikelihoodCalculator вычисляет значимость сигнала и определяет 
наилучшее значение сигнала на основе метода максимального правдоподобия. 
Возможность учета систематических эффектов также включена в калькулятор. 

\item {\it ProfileLikelihood} возможно использовать для оценки интервалов доверия. 
Возможно вычисление верхнего и нижнего пределов, а также центрального доверительного 
интервала.

\item {\it BayesianCalculator} позволяет решать задачи на основе 
метода Байеса. Причем Байесовское интегрирование может производиться численно, 
аналитически и методом Монте Карло с помощью Марковских цепей 
(MCMCCalculator - Monte Carlo Markov Chain Calculator). Здесь, конечно, очень 
важно -- выбор функции приора $\pi(\lambda)$, а также выбор интервала -- центрального  
интервала, интервала минимальной длины или одностороннего интервала. 

\item {\it HybridCalculator} вычисляет частотную вероятность событий. Учет систематики проводится 
с помощью метода Кузинса-Хайлэнда. В частности вычисляет ``п''-значения (p-value). 
Вычисления производятся с помощью Монте Карло розыгрыша псевдоэкспериментов. Также 
возможно осуществить построение Неймана (NeymanConstruction) для определения интервалов 
доверия частотным способом. Предоставляется возможность использовать несколько правил 
конструирования интервалов (интервал минимальной длины, центральный интервал, 
метод Фельдмана-Кузинса). 
Также при определении значения верхних пределов на сигнал можно использовать чисто 
$P_{sl}$ частотный подход и $CL_s=\displaystyle \frac{P_{sl}}{1-p_B}$ -- модифицированый  
частотный подход. 

\item {\it HypoTestInverter}  преобразует результат по проверке гипотез (HybridCalculator) 
в доверительный интервал (или в предел доверия) для параметра. 

\item {\it HistFactory}  обеспечивает использование статистического инструментария пакета программ 
RooStats без необходимости использовать язык моделирования данных для пакета RooFit.

\item {\it BATCalculator}. Сам пакет Байесовских вычислений с 
помощью Монте Карло цепей Маркова (BAT) является внешним к RooStats, но как класс 
в пакете программ RooStats полезен.

\end{itemize}


\subsection{Проект BAT}

BAT (the Bayesian Analysis Toolkit)~\cite{BATCPC} -- инструментарий для статистического анализа 
 также как и RooStats возник недавно. Статистический анализ 
данных в пакете программ BAT основывается на теореме Байеса и реализуется с помощью 
метода Монте Карло с использованием цепей Маркова~\cite{Markov}. Это позволяет строить апостериорные 
распределения параметров и, соответственно, проводить оценку параметров, устанавливать 
доверительные пределы и интервалы, а также осуществлять непосредственно перенос 
неопределенностей на уровне апостериорных распределений.  

Одна из главных целей анализа данных -- сравнить модельные предсказания с экспериментальными 
данными и либо сделать заключение о корректности модели по отношению к данным, либо построить 
области доверия с той или иной точностью для параметров заданной модели. 

%%\paragraph{Теоретическое обоснование}

На следующем рисунке представлена основная идея, заложенная в пакете программ BAT.\\

{\hbox{

\put(25,200){\line(1,0){100}}
\put(25,200){\line(0,1){50}}
\put(25,250){\line(1,0){100}}
\put(125,200){\line(0,1){50}}

\put(75,150){\line(0,1){50}}
\put(75,150){\line(1,1){10}}
\put(75,150){\line(-1,1){10}}
\put(80,172){Теория}

\put(275,50){\line(0,1){150}}
\put(275,50){\line(1,1){10}}
\put(275,50){\line(-1,1){10}}
\put(220,122){Обработка данных}

\put(40,230){Модель $M$}
\put(40,210){Параметры $\vec \lambda$}

\put(225,200){\line(1,0){100}}
\put(225,200){\line(0,1){50}}
\put(225,250){\line(1,0){100}}
\put(325,200){\line(0,1){50}}

\put(240,220){Эксперимент}

\put(25,100){\line(1,0){100}}
\put(25,100){\line(0,1){50}}
\put(25,150){\line(1,0){100}}
\put(125,100){\line(0,1){50}}

\put(27,135){Распределение фи-}
\put(27,120){зических величин $\vec y$}
\put(40,105){$g(\vec y|\vec \lambda, M)$}

\put(75,50){\line(0,1){50}}
\put(75,50){\line(1,1){10}}
\put(75,50){\line(-1,1){10}}
\put(80,80){Моделирование}
\put(80,70){эксперимента}

\put(25,0){\line(1,0){100}}
\put(25,0){\line(0,1){50}}
\put(25,50){\line(1,0){100}}
\put(125,0){\line(0,1){50}}

\put(27,35){Предсказание изме-}
\put(27,20){ряемых величин $\vec x$}
\put(40,5){$f(\vec x|\vec\lambda,\vec\nu,M)$}

\put(225,0){\line(1,0){100}}
\put(225,0){\line(0,1){50}}
\put(225,50){\line(1,0){100}}
\put(325,0){\line(0,1){50}}

\put(240,35){Измеренные}
\put(240,20){величины}
\put(250,5){$\vec D$}

\put(136,23){\line(1,0){75}}
\put(136,27){\line(1,0){75}}
\put(150,30){Обновление}
\put(150,13){знания}

\put(130,25){\line(1,-1){10}}
\put(130,25){\line(1,1){10}}
\put(210,35){\line(1,-1){10}}
\put(210,15){\line(1,1){10}}

}}

\bigskip

Модель $M$ может меняться от модели, описывающую природу явлений, до простой параметризации данных, 
используемой в предсказании результатов или в представлении результатов исследований. 
Теория или модель должны быть обеспечены прямыми распределениями вероятности (вероятностей 
в дискретном случае), то есть относительными частотами возможных результатов 
эксперимента, которые можно получить при многократном повторении эксперимента в идентичных 
условиях~\footnote{Термин "метод Монте-Карло" относится к моделированию процессов с использованием 
генератора случайных чисел. Термин Монте-Карло (Монте Карло это административная территория княжества 
Монако -- город известный своим казино) 
произошел из того факта, что "число шансов" (в методах моделирования Монте-Карло) было использовано 
с целью нахождения интегралов от сложных уравнений при разработке первых ядерных бомб 
(интегралы квантовой механики). С помощью формирования больших выборок случайных чисел, например, 
из нескольких распределений, интегралы этих (сложных) распределений могут быть аппроксимированы из 
(сгенерированных) данных.}. Это возможно, так как модель это математическая конструкция, которая позволяет 
вычислять (или моделировать) возможные результаты ее использования. Однако, предсказания модели 
обычно нельзя использовать напрямую для сравнения с экспериментальными данными. Нужно или модифицировать 
предсказание, чтобы учесть особенности в проведении эксперимента, или учитывать эти особенности 
при представлении результата эксперимента. Очевидно, что необходимо точное описание таких особенностей 
эксперимента, чтобы сделать надежные выводы из экспериментальных данных.

Функция $g(\vec y|\vec \lambda, M)$ описывает относительную частоту возможного результата 
$\vec y$ в рамках модели $M$ при условии наличия параметров $\vec\lambda$. При этом выполнены 
условия

\begin{equation}
g(\vec y|\vec \lambda, M) \ge 0. 
\label{eq:bat1}
\end{equation}

\noindent
Условие нормировки для дискретной величины имеет вид 

\begin{center}
$\displaystyle \sum_i{g(\vec y_i|\vec \lambda, M)}=1$,  
\end{center}

\noindent
а для непрерывной величины -- 

\begin{equation}
\int{g(\vec y|\vec \lambda, M)d\vec y}=1. 
\label{eq:bat2}
\end{equation}

Остановимся на непрерывном случае. Моделирование эксперимента добавляет в модель дополнительные 
предположения и параметры. Назовем такие параметры вспомогательными (nuisance parameters), 
хотя часто они определяют область допустимых значений основных параметров $\vec\lambda$ модели, и 
обозначим их $\vec\nu$. 


\begin{itemize}
\item[] Рассмотрим, например, радиоактивный распад нестабильных ядер. В качестве модели возьмем  
экспоненциальное распределение времени распада, то есть 
$P(t|\tau)=\displaystyle \frac{1}{\tau}e^{-\frac{t}{\tau}}$, с параметром 
времени жизни $\tau$. Пусть $\vec t=(t_1,t_2,\dots,t_n)$ -- вектор $n$ наблюдений. 
Одна из возможностей для определения $g(\vec t|\tau)$ это перемножение плотностей вероятности для 
каждого одиночного наблюдения (события) времени жизни $t_i$ -- 

$g(\vec t|\tau)=\displaystyle 
\prod_{i=1}^n{\frac{1}{\tau}e^{-\frac{t_i}{\tau}}}$.

Другая возможность определения $g(\vec t|\tau)$  -- подсчет событий (количество распадов) в  различные 
промежутки  времени и сравнение их числа с ожидаемым числом распадов, полученном из 
распределения Пуассона

$g(\vec t|\tau)=\displaystyle 
\prod_{j=1}^n{\frac{\eta_j^{k_j}}{k_j!}e^{-\eta_j}}$, 

\noindent
где $k_j$ -- число событий наблюденных в интервал времени $\Delta t_j$, 
а  $\eta_j$ -- ожидаемое число событий для этого интервала времени 

$\eta_j=\displaystyle
\int_{\Delta t_j}{\frac{N}{\tau}e^{-\frac{t}{\tau}}dt}$.

\noindent
$N$ полное число наблюденных событий.

Можно представить, что, при измерениях исследуемого образца, наш прибор не способен разделить 
два близко расположенных по времени распада, то есть имеет некоторое мертвое время. Также, 
следует предположить, что прибор имеет конечное временное разрешение. Часто полагается, что 
точность измерения времени распада распределена по нормальному закону. Параметры, описывающие 
временное разрешение и мертвое время прибора, обычно не являются параметрами, определяющими 
модель, и могут рассматриваться как вспомогательные. Тем не менее их можно учесть 
с помощью моделирования методом Монте Карло и получить для измеренной выборки 
$\vec t^{meas}=(t_1^{meas},t_2^{meas},\dots,t_n^{meas})$ плотность распределения 
величины $f(\vec t^{meas}|\tau,\sigma_t)$.

\end{itemize}

Запишем непрерывную вероятность модели $M$ как $P(M)$ со следующим свойствам

\begin{equation}
0\le P(M) \le 1 
\label{eq:bat3}
\end{equation}

\noindent  
Пусть вспомогательные параметры, описывающие условия эксперимента, не коррелируют с основными 
параметрами физической модели, то есть 

\begin{equation}
P(\vec\lambda,\vec\nu|M)=P(\vec\lambda|M)P(\vec\nu). 
\label{eq:bat4}
\end{equation}

\noindent
Пусть выполнены следующие условия:

\begin{equation}
P(\vec\lambda|M) \ge 0, 
\label{eq:bat5}
\end{equation}

\begin{equation}
\int{P(\vec\lambda|M)d\vec\lambda}=1, 
\label{eq:bat6}
\end{equation}

\begin{equation}
P(\vec\nu) \ge 0, 
\label{eq:bat7}
\end{equation}

\begin{equation}
\int{P(\vec\nu)d\vec\nu}=1. 
\label{eq:bat8}
\end{equation}

В Байесовском подходе $P(M)$ и $P(\vec\lambda|M)$ рассматриваются как плотности вероятности, 
хотя они не являются распределениями частот~\footnote{В частотном подходе они 
рассматриваются как доверительные распределения~\cite{IHEP08}.} и их следует описывать как 
распределение степени веры (degrees-of-belief)~\cite{DAgostini2003}. Это распределение 
степени веры обновляется при сравнении очередных данных эксперимента и предсказания модели, 
поправленого на результаты предыдущих измерений. Параметр и его модельное распределение 
степени веры являются предметом изучения и содержат наше знание о природе исследуемого явления. 
Целью измерений в этом смысле является модифицирование распределения степени веры. 
При этом утверждение $P(M)=1$ означает то, что модель $M$ верна, а
утверждение $P(M)=0$ означает то, что модель $M$ неверна. 

Этот построение позволяет сформулировать правило обучения в данном подходе как 

\begin{equation}
P_{i+1}(\vec\lambda,\vec\nu,M|\vec D)\propto 
f(\vec x=\vec D|\vec\lambda,\vec\nu,M)P_i(\vec \lambda,\vec\nu,M),  
\label{eq:bat9}
\end{equation}

\noindent
где индекс при $P$ обозначает текущее состояния знания. 

Из условия нормализации

\begin{equation}
\displaystyle \sum_M{\int{P(\vec\lambda,\vec\nu,M)d\vec\lambda d\vec\nu}}=
\sum_MP(M)[\int{P(\vec\lambda|M)d\vec\lambda}\int{P(\vec\nu)d\vec\nu}]=1
\label{eq:bat10}
\end{equation}

\noindent
имеем

\begin{equation}
P_{i+1}(\vec\lambda,\vec\nu,M|\vec D)= \displaystyle 
\frac{f(\vec x=\vec D|\vec\lambda,\vec\nu,M)P_i(\vec \lambda,\vec\nu,M)}
{\sum_M{\int{f(\vec x=\vec D|\vec\lambda,\vec\nu,M)P_i(\vec \lambda,\vec\nu,M)
d\vec\lambda d\vec\nu}}}.  
\label{eq:bat11}
\end{equation}

\noindent
Обычно $P_i$ называется приором и обозначается как $P_0$. Он содержит всю информацию 
о модели и значениях параметров, которой мы владеем до проведения эксперимента. Апостериорная 
вероятность $P_{i+1}$ обычно обозначается просто $P$. Она описывает состояние наших 
знаний после анализа данных эксперимента.

Для заданной модели $M$ $f$ является функцией основных параметров модели, вспомогательных 
параметров измерения и возможного результата измерений. Если $f$ зависит только от параметров 
$(\vec\lambda,\vec\nu)$ для конкретной выборки $\vec x=\vec D$, то она рассматривается как функция 
правдоподобия. В данной формулировке $f$ это относительная частота появления выборки 
$\vec x=\vec D$ при моделировании. Если $f$ нормализованы, то можно записать 

\begin{equation}
P(\vec D|\vec\lambda,\vec\nu,M)=  
f(\vec x=\vec D|\vec\lambda,\vec\nu,M)P_i(\vec \lambda,\vec\nu,M),  
\label{eq:bat12}
\end{equation}

Знаменатель в уравнении~(\ref{eq:bat11}) это вероятность получить данные $\vec D$, 
в условиях модели $M$ и параметризации эксперимента. Он описывает все возможные результаты 
эксперимента и его можно записать в виде $P(\vec D)$. В этих обозначениях 
формула~(\ref{eq:bat11}) принимает классический вид~(например,~\cite{Jaynes}) 

\begin{equation}
P(\vec\lambda,\vec\nu,M|\vec D)= \displaystyle 
\frac{P(\vec D|\vec\lambda,\vec\nu,M)P(\vec \lambda,\vec\nu,M)}{P(\vec D)}.  
\label{eq:bat13}
\end{equation}

В рамках данной модели оценка параметров осуществляется с помощью соотношения  

\begin{equation}
P(\vec\lambda,\vec\nu,|\vec D,M)= \displaystyle 
\frac{P(\vec D|\vec\lambda,\vec\nu,M)P(\vec \lambda,\vec\nu,M)}
{\int{P(\vec x=\vec D|\vec\lambda,\vec\nu,M)P_0(\vec\lambda,\vec\nu|M)}
d\vec\lambda d\vec\nu}.  
\label{eq:bat14}
\end{equation}

\noindent
Результатом оценки является нормализованная плотность вероятности параметров, 
включая все корреляции. Эта плотность позволяет строить доверительные интервалы 
для параметров, находить доверительные пределы, проверять согласованность экспериментальных 
данных и моделей и многое другое.

Апостериорная плотность вероятности~(\ref{eq:bat9}) находится методом Монте Карло,   
использующим цепи Маркова~(например,~\cite{Gilks}).

Пакет реализован на основе языка $C++$, имеет интерфейс с такими пакетами, как 
ROOT, RooStats, Minuit. Он позволяет использовать определенные пользователем 
функции и алгоритмы. 


\subsection{Многофакторные (многовариантные) методы в физике высоких энергий}

Многофакторный метод это любой статистический инструментарий, в котором заложен 
статистический анализ многомерной переменной. Основными задачами, решаемыми в таком 
анализе, являются задачи классификации объектов, аппроксимации функций, оценки плотности 
распределений, сжатия данных, отбора переменных, оптимизации, сравнения моделей и 
проверки гипотез. Рассмотрим принципы и подходы к построению данного 
инструментария~\cite{Prosper} и возможности, предоставляемые существующим 
программным обеспечением. 

Экспериментальные данные с крупных установок многомерны. Например, типичное событие рождения 
одиночного топ кварка в протон-антипротоных соударениях в конечном состоянии включает электрон  
или мюон, от двух до четырех струй адронов и потерянную поперечную энергию. 
В работе~\cite{FermiTop} 
при обнаружении рождения одиночного топ-кварка было использовано около 60 переменных и применялось 
четыре метода многофакторного анализа.  

\subsubsection{Немного теории}

Для многих приложений фундаментальную многофакторную задачу можно построить следующим 
образом: пусть существует набор обучающих данных $T=\{(y_1,x_1),(y_2,x_2), \dots\}$, где 
$y_i$ действительное (или рациональное) число в интервале $[-1,1]$ или $[0,1]$, 
а $x$ входной вектор, компоненты которого $x_i \in R^d$, и существует функция $f$ такая, 
что $y=f(x)$. Если $y$ непрерывна, 
то задачу можно назвать регрессией. Если $y$ дискретна, то говорят о задачах классификации 
или разделения. Величины $y_i$ называют целями (значениями целевой функцией) или выходным вектором, 
а величины $x_i$ входным вектором (или вектором особенности). 

Многофакторные методы можно делить по способу обучения: методы с машинным или  
с Байесовским обучением. 


\paragraph{Машинное обучение.}  

Можно выделить два типа обучения. Обучение по прецедентам, или индуктивное обучение, 
основано на выявлении закономерностей в эмпирических данных. Дедуктивное обучение предполагает 
формализацию знаний экспертов и создание базы знаний. Дедуктивное обучение принято относить 
к области экспертных систем, поэтому термины машинное обучение и обучение по 
прецедентам будем считать считать синонимами.

Рассмотрим подход к построению приближения функции $y=f(x)$ как проблему задачи оптимизации, 
то есть приближение будет результатом минимизации соответствующего функционала. 
Основные элементы анализа это:  

\begin{itemize}
\item класс параметрических функций ${\mathop{F}}=\{f(x,w)\}$, в которых 
параметры $w$ найдены при минимизации функционала;
\item ограничение $C(w)$ на класс функций ${\mathop{F}}=\{f(x,w)\}$; 
\item функция потерь $L(y,f)$, которая оценивает потери при плохом выборе функции 
$f(x,w)$ из класса функций ${\mathop{F}}=\{f(x,w)\}$. 
\end{itemize}

На практике выбранная функция $f(x,w)$ должна быть устойчива к выбору 
обучающих данных, то есть среднее значение функции потерь по обучающим данным должно 
быть минимальным (иметь лучшее значение). Это задается через функцию эмпирического риска 
$R(w)$

\begin{equation}
R(w)=\displaystyle \frac{1}{N}\sum_{i=1}^N{L(y_i,f_i)},   
\label{eq:bay1}
\end{equation}

\noindent
где $f_i=f(x_i,w)$, а $N$ -- объем выборки обучающих данных. Практической задачей 
здесь является минимизация функции эмпирического риска $R(w)$ при наличии ограничения $C(w)$, 
то есть функционала 

\begin{equation}
E(w)=R(w)+\lambda C(w),   
\label{eq:bay2}
\end{equation}

\noindent
где $\lambda$ -- параметр настройки, который определяет серьезность ограничения. 
При минимизации $E(w)$ будет выбрана функция $f(x,w*)$, которая в пределе при  
$N\rightarrow\infty$ сходится в выбранной метрике 
к функции минимизирующей риск через функцию потерь 
$L(y,f)$. Хорошо известный пример эмпирической минимизации риска это $\chi^2$ фитирование 
(подгонка) с ограничениями. 

\paragraph{Байесовское обучение.}  

В байесовском обучении исходя из полученных данных вычисляется вероятность каждой 
гипотезы и на основании этого делаются предсказания, то есть предсказания составляются 
с использованием всех гипотез, взвешенных по их вероятностям, а не с применением только одной 
"наилучшей" гипотезы. Таким образом, обучение сводится к вероятностному выводу. Это требует 
наличия 

\begin{itemize}
\item класса параметрических функций ${\mathop{F}}=\{f(x,w)\}$, в которых 
параметры $w$ находятся минимизацией функционала;
\item плотности приора $\pi(f)$ по пространству функций, хотя на практике используют 
более простой путь определения приора по пространству параметров;
\item функции правдоподобия $p(y|x,w)$ пропорциональной вероятности того, что 
величина функции $f(x)$ будет равна $y$ при заданном входе $x$. 
\end{itemize}

Преимущество Байесовского подхода в том, что все интерференционные проблемы 
решаются одним способом~\cite{Hagan}. Проблема состоит в том, чтобы определить вероятные значения 
параметров $w$, и, следовательно, сделать вероятностный выбор функции $f(x,w)$, учитывая обучающие
данные $T$. Это делается вычислением апостериорной вероятности $p(w|T)dw$, 
то есть вероятности того, что выбор $w$ совместим с обучающими данными $T$. 
Стандартный способ произвести это вычисление состоит в использовании теоремы Байеса 

\begin{center}
$p(w|T)=\displaystyle \frac{p(T|w)\pi(w)}{p(T)}$   
\end{center}

\begin{center}
$~~~~~~=\displaystyle \frac{p(y,x|w)\pi(w)}{p(y,x)}$   
\end{center}

\begin{center}
$~~~~~~=\displaystyle \frac{p(y|x,w)p(x|w)\pi(w)}{p(y|x)p(x)}$   
\end{center}

\begin{equation}
~~~~~\sim\displaystyle p(y|x,w)\pi(w),   
\label{eq:bay3}
\end{equation}

\noindent
здесь мы делаем разумное предположение, что $p(x|w)=p(x)$ потому, что плотность вероятности 
входного вектора $x$ не зависит от параметров функции, которая будет получена.   
Функция $p(w|T)dw$ определяет значение функции $f(x,w)$ в соседнем с точкой $w$ отрезке 
$[w, w+dw]$. Большие значения $p(w|T)$ подразумевают, что функция $f(x,w)$ лучше согласована  
с обучающими данными.

В рамках Байесовского подхода~\cite{Hagan} данная апостериорная плотность $p(w|T)$ позволяет 
вычислить прогнозирующее распределение

\begin{equation}
p(y|x,T)=\int{p(y|x,w)p(w|T)dw},   
\label{eq:bay4}
\end{equation}
 
\noindent
то есть плотность вероятности того, что функция принимает значение $y$ при данном значении 
входного вектора $x$. Часто используют точечную оценку значения $y = f(x)$. Она может быть 
получена при минимизации функции риска

\begin{equation}
y=\displaystyle arg_y min \int{L(z,y)p(z|x,T)dz},   
\label{eq:bay5}
\end{equation}

\noindent
где $L(z,y)$ некоторая функция потерь. Здесь минимизируются квадратичные 
потери, задаваемые как 

\begin{equation}
L(a,b)=(a-b)^2.    
\label{eq:bay6}
\end{equation}

При таком выборе вида функции потерь оптимальная оценка значения функции $y = f(x)$ определяется как 
среднее прогнозирующего распределения 

\begin{equation}
y=\int{zp(z|x,T)dz},   
\label{eq:bay7}
\end{equation}

\paragraph{Сравнение машинного и Байесовского обучения.}  

Хотя рассмотренные подходы различны, они не так различаются, как кажутся. 
Если мы рассмотрим следующие тождества 

\begin{center}
$R(w) \sim ln{~p(y|x,w)}$,   
\end{center}

\begin{equation}
~~~~~= \displaystyle \sum_{i=1}^N{ln{~p(y_i|x_i,w)}},   
\label{eq:bay8}
\end{equation}

\begin{equation}
\lambda C(w) \sim ln{~\pi(w)},   
\label{eq:bay9}
\end{equation}

\noindent
то становится ясно, что машинный подход обучения может быть рассмотрен как обеспечение Максимума
АПостериорной (МАП) оценки функции $y = f(x)$, то есть при нахождении наилучшей оценки $f(x,w*)$ функции 
$y=f(x)$ задача минимизации эмпирического риска с ограничениями~(\ref{eq:bay2}) эквивалентна 
максимизации апостериорной плотности~(\ref{eq:bay3}). В то время как в Байесовском подходе 
процедура присваивает определенную вероятность всем возможным выборам функции $f(x,w)$.

\paragraph{Регрессия и классификация.}  

Регрессия (например, подгонка кривой) и классификация отличаются
выбором целей $y$ и функциями потерь $L$. 

В случае регрессии цели это непрерывные функции входных данных, а функцией потерь, 
обычно, считаются квадратичные потери~(\ref{eq:bay6}). Этот 
выбор приводит к следующей функции эмпирического риска 

\begin{equation}
\lambda R(w) = \displaystyle\frac{1}{N}\sum_{i=1}^N{(y_i-f(x_i,w))^2},   
\label{eq:bay10}
\end{equation}

\noindent
или, что эквивалентно, к функции правдоподобия 

\begin{equation}
p(y|x,w)=\displaystyle \frac{1}{\sqrt{2\pi}\sigma}e^{-\frac{NR(w)}{2\sigma^2}}.   
\label{eq:bay11}
\end{equation}


Для классификации лучший выбор для функции правдоподобия (и, следовательно, 
функции эмпирического риска)

\begin{equation}
p(y|x,w)=\displaystyle 
\prod_{i=1}^N{f(x_i,w)^{\omega_iy_i}[1-f(x_i,w)]^{\omega_i(1-y_i)}},   
\label{eq:bay12}
\end{equation}

\noindent
где $0<f(x_i,w)<1$, а значения целевой функции $y_i$ принимают дискретные значения $0$ и $1$. 
При классификации $f(x,w)$ интерпретируется как вероятность того, что входной вектор $x$ 
принадлежит классу значений целевой функции $y=1$. В уравнении~(\ref{eq:bay12}) 
вводятся дополнительные веса $\omega_i$ для каждой компоненты (или особенности) входного 
вектора $x_i$. В физике частиц в методе Монте Карло модели обычно взвешиваются пособытийно, чтобы 
откорректировать недостатки моделирования.  Соответствующей функцией 
эмпирического риска является 

\begin{equation}
R(w)=\displaystyle 
\frac{1}{N}\sum_{i=1}^N{\omega_i[y_ilnf(x_i,w)+(1-y_i)ln(1-f(x_i,w))]}.
\label{eq:bay13}
\end{equation}

Показано~(например,~\cite{Bishop}), что оптимальный выбор значения функции $f(x,w)$ это тот, который 
аппроксимирует вероятность $p(1|x)$ так, что входной вектор $x$ принадлежит классу 
помеченному 1 

\begin{equation}
p(1|x)=\displaystyle 
\frac{p(x|1)p(1)}{p(x|1)p(1)+p(x|0)p(0)}, 
\label{eq:bay14}
\end{equation}

\noindent
где $p(1)$ и $p(0)$ -- априорные вероятности для классов, помеченных 
соответственно $1$ и $0$, а $p(x|1)$ и $p(x|0)$ -- соответствующие плотности вероятности 
для входных векторов. В задачах разделения сигнала и фона, класс ``сигнал'' обычно 
помечается $1$, а класс ``фон'' -- соответственно $0$ (иногда даже $-1$). В данном 
случае отношение $\displaystyle \frac{p(1)}{p(0)}$ будет априорным отношением 
сигнал/фон. 

Для заданной вероятности $p(1|x)$ можно определить Байесовский классификатор: 

\underline{\bf Байесовский классификатор:} Если $p(1|x)>q$, то $x$ считается 
принадлежащим классу, помеченным $1$, где величина $q$ является порогом, выбранным 
для анализа~\footnote{Формально, этот выбор определяется минимизацией выбранной функции потерь.}.

Байесовский классификатор оптимален в том смысле, что при его использовании достигается 
наименьший процент ложных отбраковок. Например, если цель состоит в том, чтобы различить
электроны и файкэлектроны (при ложной идентификации частицы как электрона)  
и сделать это с наименьшим количеством ошибок, тогда нужно использовать Байесовский классификатор. 
На практике обычно неизвестны априорные вероятности $p(1)$ и $p(0)$. Часто это именно то, что 
необходимо измерить. Поэтому кажется, что нельзя использовать Байесовский классификатор. 
Но это не так. Для классификации достаточно аппроксимировать дискриминант

\begin{equation}
D(x)=\displaystyle 
\frac{p(x|1)}{p(x|1)+p(x|0)}, 
\label{eq:bay15}
\end{equation}

\noindent
потому, что $D(x)$ и $p(1|x)$ связаны взаимооднозначным соответствием 

\begin{equation}
p(1|x)=\displaystyle 
\frac{D(x)}{D(x)+\frac{1-D(x)}{A}}, 
\label{eq:bay16}
\end{equation}

\noindent
где $A=\displaystyle \frac{p(1)}{p(0)}$. Классификация с использованием $D(x)$ с 
заданным порогом эквивалентна классификации с использованием $p(1|x)$ с неизвестным 
порогом. 

Функция $p(1|x)$ оптимальна в другом смысле~\cite{Barlow2}. Если веса в 
смеси сигнальных и фоновых событий определяются весовой функцией $W(x)=p(1|x)$, то 
доля сигнала может быть оценена с нулевым смещением и минимальной дисперсией при условии, 
что зависимость веса от $x$ может быть точно смоделировано и отношение $A$ равно 
истинному значению. Так как мы не знаем истинного значения $A$, то, вероятно, можно 
построить итеративную процедуру сходящуюся к $A$. Оптимальность Байесовского классификатора 
зависит от решаемой задачи. Например, если нужно классифицировать объекты с наименьшим 
количеством ошибок, то он оптимален, если же нужно измерить массу Хиггса с минимальной 
неопределенностью, то Байесовский классификатор не обязательно оптимален.
  
\subsubsection{Многофакторные методы на практике}

Для важной задачи разделения сигнал/фон существует большое количество многофакторных методов.  
Приведем неполный список этих методов.

\begin{itemize}

\item  {\bf Линейные и  Нелинейные Дискриминанты} 
({\it Linear and Nonlinear Discriminants}).
Дискриминантный анализ это раздел вычислительной математики, представляющий основное средство 
решения задач распознавания образов, инструмент статистики, который используется для принятия 
решения 
о том, какие переменные разделяют возникающие наборы данных. \\  

\item  {\bf Метод опорных векторов} ({\it Support Vector Machines}). 
Это набор схожих алгоритмов вида ``обучение с учителем'', использующихся для задач 
регрессионного анализа
и классификации~\cite{Vapnik}. \\ 

\item  {\bf Дискриминант Правдоподобия} ({\it Likelihood Discriminant}). 
Примитивный (наивный) байесовский классификатор -- 
простой вероятностный классификатор, основанный на применении теоремы Байеса со строгими (наивными) 
предположениями о независимости~\cite{Subbotin}.

\item  {\bf Ядерная Оценка Плотности} ({\it Kernel Density Estimation}). 
В статистике ядерная оценка плотности это непараметрический способ оценить функцию плотности 
вероятности 
случайной переменной~\cite{Orlov}.  \\

\item  {\bf Нейронные сети}  ({\it Neural Networks}). 
Искусственные нейронные сети -- математические модели, а 
также их программные или аппаратные реализации, построенные по принципу организации и 
функционирования 
биологических нейронных сетей -- сетей нервных клеток живого организма. Это понятие возникло 
при изучении 
процессов, протекающих в мозге, и при попытке смоделировать эти процессы. Впоследствии, после 
разработки 
алгоритмов обучения, получаемые модели стали использовать в практических целях: в задачах 
прогнозирования, 
для распознавания образов, в задачах управления и др.~\cite{Haikin}. Один из наиболее простых и,
тем не менее, широко применяемых типов нейросетей -- многослойный персептрон.  
Многослойными персептронами называют нейронные сети прямого распространения. Входной сигнал в 
таких сетях 
распространяется в прямом направлении, от слоя к слою. Многослойный персептрон в общем 
представлении состоит 
из следующих элементов:

\begin{itemize}
   \item множества входных узлов, которые образуют входной слой;
   \item одного или нескольких скрытых слоев вычислительных нейронов;
   \item одного выходного слоя нейронов. 
\end{itemize}
Многослойный персептрон представляет собой обобщение однослойного персептрона 
Розенблатта~\cite{Rosenblatt}. Основным элементом нейронной сети является нейрон, который 
имеет один или несколько входов и один выход, значение которого вычисляется через передаточную 
функцию (или функцию активации нейрона). Если два нейрона по обе стороны синапса (соединения) 
активизируются одновременно (то есть синхронно), то прочность этого соединения возрастает. Если 
два нейрона по обе стороны синапса активизируются асинхронно, то такой синапс ослабляется или 
вообще отмирает. 

Важным свойством любой нейронной сети является способность к обучению. Классический метод обучения 
перцептрона -- это метод коррекции ошибки. Он представляет собой вид обучения с учителем, 
при котором вес связи не изменяется до тех пор, пока текущая реакция перцептрона остается правильной. 
При появлении неправильной реакции вес изменяется на единицу, а знак (+/-) определяется противоположным 
от знака ошибки. Существует метод Розенблатта обучения без учителя, а также градиентные методы 
(например, метод обратного распространения ошибки~\cite{Galushkin,Rumelhart}). \\ 

\item  {\bf Байесовские нейронные сети} ({\it Bayesian Neural Networks}). 

Если методы построения и обучения нейронных сетей являются Байесовскими, то и сети называются 
Байесовскими нейронными сетями. Существуют два подхода к Байесовскому обучению нейронных сетей -- 
подход МакКея~\cite{MacKay} и Нила~\cite{Neal}. В физике высоких энергий под Байесовскими 
сетями обычно понимают сети с обучением по второму подходу. Байесовские нейросети имеют ряд черт 
качественно отличающих их от нейронных сетей в традиционном подходе. Для них не 
осуществляется градиентный поиск минимума ошибки, то обучения в его классическом понимании 
не производится. Тем не менее, из-за использования в методе 
Монте Карло Марковских цепей, при применении   
Байесовских нейросетей необходимы значительные вычислительные ресурсы. Результатом обучения 
нейросети является не одна ``натренированная'', то есть обученная, сеть, а ансамбль, обычно 
содержащий сотни сетей. Все эти сети имеют одинаково большое 
число нейронов в скрытом слое.  \\ 

\item  {\bf Деревья принятия решений} ({\it Decision Trees}). 
Деревья принятия решений обычно используются 
для решения задач классификации данных или, иначе говоря, для задачи аппроксимации заданной булевой 
функции. Ситуация, в которой стоит применять деревья принятия решений, обычно выглядит так: 
есть много случаев, каждый из которых описывается некоторым конечным набором дискретных атрибутов, 
и в каждом из случаев дано значение некоторой (неизвестной) булевой функции, зависящей от этих атрибутов. 
Задача -- создать достаточно экономичную конструкцию, которая бы описывала эту функцию и позволяла бы  
классифицировать новые, поступающие извне данные. Дерево принятия решений это дерево, на ребрах которого 
записаны атрибуты, от которых зависит целевая функция, в листьях записаны значения целевой функции, а в 
остальных узлах -- атрибуты (признаки), по которым различаются случаи. Чтобы классифицировать новый случай, 
надо спуститься по дереву до листа и выдать соответствующее значение~\cite{Levitin}.  \\ 

\item  {\bf Случайные Леса} ({\it Random Forests}). Алгоритм машинного обучения заключается в 
использовании ансамбля решающих деревьев. Алгоритм сочетает в себе метод бэггинга 
(Bootstrap AGGregating -- объединения выборок) и метод случайных подпространств. 
Алгоритм применяется для задач классификации, регрессии и кластеризации~\cite{Hastie}. \\ 

\item {\bf Генетические алгоритмы} ({\it Genetic algoritms}). 
Генетический алгоритм это эвристический 
алгоритм поиска, используемый для решения задач оптимизации и моделирования путём случайного подбора, 
комбинирования и вариации искомых параметров с использованием механизмов, напоминающих биологическую 
эволюцию~\cite{Holland}.

\end{itemize}

Можно также отметить  Случайный Поиск по Сетке (Random Grid Search), который позволяет 
обойти трудности, возникающие при использовании регулярных сеточных алгоритмов. 

Часть из перечисленных методов реализована в пакете программ TMVA~\cite{TMVA}.

\paragraph{TMVA - инструментарий для многофакторного анализа (the Toolkit for
Multivariate Analysis)}.

Многофакторные методы классификации, основанные на методах машиного обучения, играют 
в настоящее время 
фундаментальную роль в исследованиях физики высоких энергий. При постоянно возрастающих объемах 
данных и усложнении установок, производящих эти данные, становится важным использовать 
все возможные проявления в экспериментальных данных сигнальных и фоновых событий. Анализ событий 
становится многомерным с очень большим количеством размерностей, часто коррелированных. 
TMVA~\cite{TMVA} - набор инструментов, которые позволяют реализовать большое разнообразие 
многофакторных   
алгоритмов классификации. В частности, в программе задействованы следующие классификаторы: 

\begin{itemize}
\item оптимизация линейных обрезаний; 
\item проекционное оценивания методом максимального правдоподобия; 
\item многомерное оценивание методом максимального правдоподобия; 
\item линейный и нелинейный дискриминантный анализ; 
\item искусственные нейронные сети; 
\item метод опорных векторов; 
\item усиленные (boosted) деревья принятия решений и деревья с бэггингом (bagging)~\footnote{Метод определения характеристик с помощью 
бутстреп размножения выборок и определения средних величин.}; 
\item прогнозирующее обучение через ансамбли правил (via rule ensembles). 
\end{itemize}

Пакет также позволяет организовать решение следующих задач:

\begin{itemize}
\item нахождение зависимостей между данными (задачи регрессии); 
\item классификация множества классов;
\item автоматической настройки классификаторов и их проверка с помощью взаимотестирования; 
\item усиление (бустинг) и бэггинг как собственные характеристики классификатора; 
\item составные классификаторы для параллельного, но независимого обучения различных 
областей фазового пространства; 
\item комбинированное преобразование входных данных; 
\item параллельная (multi threaded) минимизация и обучение классификатора. 
\end{itemize}

\paragraph{Пакет SPR (StatPatternRecognition)} 

Пакет SPR~\cite{SPR} обеспечивает пользователя доступом к методам многовариантного анализа. 
Анализ для выбранного классификатора состоит из обучения и тестирования. На стадии обучения 
пользователь создает тренируемый классификатор и обучает его за определенное число циклов 
или поставкой параметров для этого классификатора из работающего модуля в SPR, 
или при использовании 
соответствующего интерфейса (SprRootAdapter) из интерактивной сессии ROOT~\cite{ROOT}. 
Для классификатора, который требует больше, чем один учебный цикл, можно контролировать 
поток ошибок классификатора, благодаря специальным тестовым данным. После того, 
как обучение закончено,
можно сохранить конфигурацию обученного классификатора в системе. 
В любое время можно восстановить сохраненную конфигурацию и либо продолжить обучение, либо 
использовать классификатор для задачи классификации данных. 

Дерево принятия решений в пакете программ~\cite{Breiman} состоит из двух составляющих -- 
регулярное дерево принятия решений и нисходящее дерево решений, что позволяет ускорять процедуру 
принятия решения в задачах различной сложности. 

Алгоритм ``охотника за пиками''~\cite{Friedman} позволяет оптимизировать некоторую меру (например, 
значимость превышения сигнала над фоном) и находить в многомерном пространстве многогранник с 
наилучшим потенциалом на открытие. 

Усиление (boosting~\cite{Freund}) работает, добавляя много слабых классификаторов последовательно и 
увеличивая веса неправильно классифицированных событий на каждом шаге. Фокусируясь на событиях, 
которые являются неправильно классифицированными большую часть времени, усиление как правило достигает 
очень хорошей прогнозирующей степени.

Бэггинг (the bagging) алгоритм~\cite{Breiman2}, который находит среднее по многим слабым классификаторам, 
построенным как бутстрап копии обучающего набора данных. SPR позволяет использовать бэггинг 
для произвольной последовательности классификаторов. Усредненные деревья решений используются в 
исследованиях с машинным обучением и применяются в физическом анализе. 

Случайный лес~\cite{Breiman3} как правило используется в соединении с бэггингом и представляет 
собой набор деревьев принятия решений. Каждое дерево построено, используя случайно отобранные входные 
переменные для каждого выбора решения. Случайное осуществление выборки входных переменных уменьшает 
корреляцию среди деревьев принятия решений и улучшают полную мощность классификатора.

SPR осуществляет прямую связь с обратным переносом в нейронной сети с логистической функцией 
активации~\cite{Haikin}. 

SPR также позволяет использовать ряд дополнительных инструментов для анализа данных~\cite{Narsky2}.

\paragraph{Среда для принятия решений по выбору и уменьшению числа переменных PARADIGM.}

В физике высоких энергий выбор и уменьшение числа переменных в многофакторном анализе играет 
важную роль, поскольку, например, начальный выбор переменных часто приводит к наборам переменных 
с очень большим количеством составляющих. Иногда большим, чем количество степеней свободы основной 
модели. Это обуславливает потребность в обоснованном сокращении количества переменных. Примером одного 
из решений данной проблемы является среда для самосогласованного принятия решений по выбору и уменьшению 
число переменных PARADIGM~\cite{PARADIGM}. Решение о судьбе переменной в данной системе программ 
основывается на некоторой мере, называемой глобальной функцией потерь. В системе также определяется 
количественное значение такого свойства, как ``важность`` каждой переменной, позволяющего выделить 
наиболее существенные переменные в применяемой модели. 


\subsection{Организационная база развития статистических методов и программных средств 
анализа экспериментальных данных}\

Достаточно долго существуют Рабочая группа по статистики в Коллаборации
BaBar~\cite{BaBar} и Комитет по статистики в коллаборации CDF~\cite{CDF}. 
Основной задачей этих комитетов является выработка рекомендаций и 
стандартов в использовании Коллаборациями статистических методов обработки 
данных. 

Физиками было проведено несколько специальных Рабочих Совещаний и 
Конференций с целью унификации методов анализа и представления
конечных данных с экспериментов: 
Workshop on confidence limits, CERN, January, 2000~\cite{CL2000}, 
Workshop on confidence limits, Fermilab, March, 2000~\cite{FNAL2000}, 
Conference ``Advanced Statistical Techniques in Particle Physics'',
Durham, March, 2002~\cite{Durham}, 
Conference PHYSTAT2003, SLAC, September, 2003~\cite{SLAC}, 
Conference PHYSTAT2005, Oxford, September, 2005~\cite{Oxford}.

Всвязи с подготовкой к началу и с началом работы LHC заметно возросла 
исследовательская деятельность в области статистики. Были созданы специальные
структуры: Статистический комитет CMS~\cite{CMSCom}, 
Объединенный статистический форум ATLAS-CMS~\cite{ATLCMS}. 
Было организовано несколько рабочих совещаний, посвященные запуску LHC,  
PhyStat-LHC  Workshop, CERN, June, 2007~\cite{PLHC} и 
ACAT'2008, Are we ready for LHC era experiments?, Erice, 
November, 2008~\cite{ACAT08}, а также очередное совещание   
PhyStat'2011, CERN, January, 2011~\cite{PhyStat11}.



%тогда становится ясно, что машинный подход изучения может быть рассмотрен как обеспечение максимума
%по опыту (КАРТА) оценка функции y = f (x). Другими словами, уменьшение принужденного
%эмпирический риск, Eq. (2.2), эквивалентно максимизированию следующей плотности, Eq. (2.3), чтобы найти сингл
%наилучшая оценка f (x; w) функции y = f (x), в то время как в Байесовском подходе каждый назначает a
%вероятность ко всему возможному выбору для f (x; w).


